Iterative Neural Autoregressive Distribution Estimator (NADE-k)

Training of the neural autoregressive density estimator (NADE) can be viewed as doing one step of probabilistic inference on missing values in data. We propose a new model that extends this inference scheme to multiple steps, arguing that it is easier to learn to improve a reconstruction in $k$ steps rather than to learn to reconstruct in a single inference step. The proposed model is an unsupervised building block for deep learning that combines the desirable properties of NADE and multi-predictive training: (1) Its test likelihood can be computed analytically, (2) it is easy to generate independent samples from it, and (3) it uses an inference engine that is a superset of variational inference for Boltzmann machines. The proposed NADE-k is competitive with the state-of-the-art in density estimation on the two datasets tested.

==> Makefile <==
PAPER = nade-k

all: ${PAPER}.pdf

${PAPER}.pdf: ${PAPER}.tex myref.bib plots_for_paper/* plots_for_paper/2h/* main.tex
	pdflatex ${PAPER}.tex
	bibtex $(PAPER)
	pdflatex ${PAPER}.tex
	pdflatex ${PAPER}.tex
clean:
	rm -f ${PAPER}.aux ${PAPER}.blg ${PAPER}.pdf ${PAPER}.log ${PAPER}.out \
	    ${PAPER}.nav


